Multiple-Play Bandits in the Position-Based Model

Sequentially learning to place items in multi-position displays or lists is a task that can be cast into the multiple-play semi-bandit setting. However, a major concern in this context is when the system cannot decide whether the user feedback for each item is actually exploitable. Indeed, much of the content may have been simply ignored by the user. The present work proposes to exploit available information regarding the display position bias under the so-called Position-based click model (PBM). We first discuss how this model differs from the Cascade model and its variants considered in several recent works on multiple-play bandits. We then provide a novel regret lower bound for this model as well as computationally efficient algorithms that display good empirical and theoretical performance.

==> related.tex <==
%!TEX root = nips.tex
%

%\section{Related Work}
%\label{sec:related}
\hl{[Much of this section actually lies in the Introduction... must be shorter 
and refer to different work.]}


The $L$-best arms problem with semi-bandit 
feedback has been considered by 
\cite{anantharam1987asymptotically} who obtained a lower bound on the regret 
as 
well as an asymptotically optimal -- but computationally inefficient -- 
algorithm. The recent work by \cite{komiyama2015optimal} suggests and 
analyzes an efficient policy based on Thompson Sampling 
\cite{thompson1933likelihood} whose regret is proven asymptotically optimal.


Several recent works have considered the so called \emph{Cascade Model}
\cite{kveton2015cascading,kveton2015combinatorial,combes2015learning}. This
model comes from the Information Retrieval (IR) literature and postulates that
the user scans the proposed list of items from top to bottom and clicks on the
first interesting item, stopping at this position. It appears
highly unrealistic in on-line advertising settings where the user is not making
queries to obtain information but is proposed content she did not ask
for. Under the cascade model, it is easily checked as well that any permutation 
of the
list of $L$ optimal arms is also optimal. Hence, this model does not enforce the
necessity of ranking the items shown in the list. Indeed,
there are clear indications that the optimal strategy consists in showing the 
most relevant items at the end of the list in order to
maximize the amount of observed feedback \cite{kveton2015cascading} -- which is 
again counter-intuitive in the recommendation context.

To overcome these limitations, \cite{combes2015learning} introduce weights --
to be defined by the learner -- that are attributed to positions in the list,
with a click on position $l \in \{1,\dots,L\}$ providing a reward $r(l)$, where
the sequence $(r(l))_l$ is decreasing to enforce the ranking behavior. The
authors propose an algorithm based on KL-UCB \cite{garivier11} and prove a
lower bound on the regret as well as an asymptotically optimal upper bound.

Some preliminary considerations about the VA model can be found in the
appendix of the work by \cite{komiyama2015optimal}, where it is suggested to
model the feedback received beyond the first click in the cascade model. We
provide below a lower bound for the D-VA model as well as
algorithms that are more reliable than the variant of Thompson sampling
proposed by \cite{komiyama2015optimal} to handle this model.


